Non-Negative Matrix Factorization for Event Data

Continuous-time event data, in which entities emit instantaneous events over time, arises naturally across many domains such as neuroscience, seismology, and social networks. Non-negative matrix factorization (NMF) is a natural tool to uncover interpretable structure in such data, but it has so far only been applied after binning or smoothing the entity-level counting measures. This preprocessing step comes with the risk of erasing entity-level heterogeneities and fine-grained temporal features. In this paper, we introduce EventNMF, a continuous-time non-negative factorization model that operates directly on event times: each entity's events are modeled as a Poisson process whose intensity factorizes through a non-negative B-spline basis, and a simple estimation procedure recovers interpretable temporal templates shared across entities. The resulting method is mathematically principled, easy to implement, and computationally efficient. We further show that standard binned-count approaches arise as the special case of degree-zero splines, explore bias-variance tradeoffs and compare against existing methods on a synthetic latent factor model, and demonstrate the effectiveness of EventNMF on several real-world applications.

==> temporal_network.tex <==
\subsection{Temporal Networks}

We apply EventNMF to the SocioPatterns high-school contact dataset~\citep{fournetContactPatternsHigh2014},
recording $9{,}957$ face-to-face interactions among 156 students from 5 classes over one school day.
Following~\citet{gauvinDetectingCommunityStructure2014}, contacts are symmetrised and the pairwise intensity
is modelled as $\lambda_{ij}(t) = \sum_r U_{ir}V_{jr}f_r(t)$ with a histogram basis ($K=50$ bins, $R=13$),
making EventNMF a continuous-time generalisation of non-negative tensor factorisation (NTF).
\Cref{fig:hs-factors} shows hard-assignment membership ($\operatorname{argmax}_r U_{ir}$) sorted by factor:
several factors align predominantly with a single ground-truth class (\textit{PSI*}, \textit{MP*2}, \textit{PC}),
reproducing the community structure of~\citet{gauvinDetectingCommunityStructure2014};
a cubic spline basis recovers the same structure with smoother temporal profiles.


\begin{figure*}
  \centering
  % ── Row: three panels with tuned widths ──────────────────────────────────
  \begin{subfigure}[t]{0.26\textwidth}
    \includegraphics[width=\textwidth]{figures/highschool/fig_hs_embeddings.pdf}
    \caption{t-SNE of student embeddings $W_i$, coloured by
      ground-truth class. Students from the same class cluster
      together, recovering community structure without supervision.}
    \label{fig:hs-embeddings}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.22\textwidth}
    \includegraphics[width=\textwidth]{figures/highschool/fig_hs_affinity.pdf}
    \caption{Class--factor affinity matrix. Each row is normalised;
      dark cells indicate a factor dominated by that class
      (\textit{PSI*}, \textit{MP*2}, \textit{PC}).}
    \label{fig:hs-affinity}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.48\textwidth}
    \includegraphics[width=\textwidth]{figures/highschool/fig_hs_factors.pdf}
    \caption{Temporal factor profiles $f_r(t)$, coloured by dominant
      class. Flat profiles reflect sustained within-class contact
      during lessons; peaked profiles correspond to free-mixing
      periods (breaks, lunch).}
    \label{fig:hs-profiles}
  \end{subfigure}

  \caption{%
    EventNMF on the SocioPatterns Primary School dataset
    ($R=13$, B-spline basis of degree $3$ with $B=50$ knots).
    Factors align with ground-truth classes~\citep{gauvinDetectingCommunityStructure2014}
    and their temporal profiles distinguish lesson-time interaction
    from free-period mixing.}
  \label{fig:hs-factors}
\end{figure*}
